Green-PoW: An Energy-Efficient Blockchain Proof-of-Work Consensus Algorithm

This paper opts to mitigate the energy-inefficiency of the Blockchain Proof-of-Work (PoW) consensus algorithm by rationally repurposing the power spent during the mining process. The original PoW mining scheme is designed to consider one block at a time and assign a reward to the first place winner of a computation race. To reduce the mining-related energy consumption, we propose to compensate the computation effort of the runner(s)-up of a mining round, by granting them exclusivity of solving the upcoming block in the next round. This will considerably reduce the number of competing nodes in the next round and consequently, the consumed energy. Our proposed scheme divides time into epochs, where each comprises two mining rounds; in the first one, all network nodes can participate in the mining process, whereas in the second round only runners-up can take part. Thus, the overall mining energy consumption can be reduced to nearly $50\%$. To the best of our knowledge, our proposed scheme is the first to considerably improve the energy consumption of the original PoW algorithm. Our analysis demonstrates the effectiveness of our scheme in reducing energy consumption, the probability of fork occurrences, the level of mining centralization presented in the original PoW algorithm, and the effect of transaction censorship attack.

==> fork_plot.tex <==
\begin{figure}
\centering
  \begin{tikzpicture}
      \begin{axis}[domain=0:12,xmin=0,xmax=12,ymin=0,ymax=1]
        \addplot[red,smooth] {(1-(0.9983^x))*10};
      \end{axis}
  \end{tikzpicture}
 \caption{Caption}
 \label{fig:fork:plot}
\end{figure}

==> notes.tex <==
-Why only select miner for the second round, why not determine miners for the  3rd, 4th, etc. round?
--> answer: (1) it is hard to ensure that all nodes in the network will achieve a consensus about the order of winners. Also, (2) by knowing the subset of miners that are concerned by mining in the next 3rd, 4th,.. round, an attacker will have enough time to plan for a strategic way to isolate that nodes by attacking them directly or by monitoring their outbound traffic .
--------

How to mitigate to the case when a very very small subset of second place winner are selected, and for any reason they will not process to mining in the second round? (Finality problem, cash payment ensure immediate finality, whereas bitcoin ensure probabilistic finality)  


% By design, Green-PoW reduces the total network hashrate during the second round. So, maintaining the same level of mining difficulty for both rounds will yield to inconsistencies in the block generation time. To ensure a constant block time during both mining rounds, we define a new difficulty adjustment scheme which uses two difficulties instead of one, namely $D_1$ and $D_2$. The network shifts between them depending on the current mining round. Both difficulties are calculated based on the original approach discussed in section 3.1.2, however $D_1$ considers blocks that are tagged with $D_1$ solely when calculating the average block time of the previous difficulty period (equation \ref{eq:3}). Where as $D_2$ (equation \ref{eq:4}), considers the ones tagged with $D_2$.This change in design grants network adaption to the huge drop in the hashing rate of the second round. In the case of second round timeout, the network will switch back to $D_1$, to avoid forks occurrence caused by the inadequate difficulty level compared to the total hashrate. 
% \begin{equation}\label{eq:3}
% D'_{1}= D_{1}\times \dfrac{T_{E}}{(\sum_{k=1}^{1008} T_{D1}(k))/1008} 
% \end{equation}
% \begin{equation}\label{eq:4}
% D'_{2}= D_{2}\times \dfrac{T_{E}}{(\sum_{k=1}^{1008} T_{D2}(k))/1008} 
% \end{equation}
% \begin{equation}\label{eq:3}
% D'_{1}= D_{1}\times \dfrac{Bt_{E}}{(\sum_{k=2i}^{2016} Bt_{k})/1008} 
% \end{equation}
% \begin{equation}\label{eq:4}
% D'_{2}= D_{2}\times \dfrac{Bt_{E}}{(\sum_{k=2i+1}^{2015} Bt_{k})/1008} 
% \end{equation}


\begin{comment}
\section{System overview}
\subsection{Basic idea}
Our goal is to propose an energy efficient  PoW consensus algorithm without affecting its security level.  To understand the idea, we first describe in the following how PoW reaches consensus and why it consumes such huge amount of electricity. As shown in \figurename \ref{fig:original_bitcoin}, each Bitcoin node, for every new block, starts the mining process by looking for the nonce that solve the block-related puzzle. The first node that founds the nonce is considered as the leader for creating the new block and get rewarded of the block it announce it  to the others. Every node that receive the new block  and then release the mining of the current block and immediately start mining a new one. In Bitcoin, all the mining nodes are competing in order to be the first to find the nonce, and thus get rewarded. All the spent power by the network nodes, during one mining round, will mainly and only serve to elect the node (leader) that will be responsible of adding the immediate next  block to the blockchain.  
Our main idea consists in saving the electricity power required during mining by allowing the network to not only select one leader, but to elect two leaders that will be responsible of adding the next and also the second next block during the same mining round. For this purpose, during a mining round, after finding the nonce by the winner, and in contrast to the traditional PoW, the other miners will continue mining the current block in order to determine the potential second-place winner(s) of that block. This potential second-place winner(s) will be the node(s) responsible of mining the second next block, consequently, a huge energy amount will be saved. \figurename \ref{fig:modified_bitcoin} summaries the mining process in the new proposed PoW that we (not sure about the naming). In this new protocol...
\end{comment}
